SPAE: Semantic Pyramid AutoEncoder for Multimodal Generation with Frozen LLMs

In this work, we introduce Semantic Pyramid AutoEncoder (SPAE) for enabling frozen LLMs to perform both understanding and generation tasks involving non-linguistic modalities such as images or videos. SPAE converts between raw pixels and interpretable lexical tokens (or words) extracted from the LLM's vocabulary. The resulting tokens capture both the semantic meaning and the fine-grained details needed for visual reconstruction, effectively translating the visual content into a language comprehensible to the LLM, and empowering it to perform a wide array of multimodal tasks. Our approach is validated through in-context learning experiments with frozen PaLM 2 and GPT 3.5 on a diverse set of image understanding and generation tasks. Our method marks the first successful attempt to enable a frozen LLM to generate image content while surpassing state-of-the-art performance in image understanding tasks, under the same setting, by over 25%.

==> sections/3_method_bk.tex <==
\vspace{-3mm}
Our goal is to model a foreign modality (\eg, image, video, and audio) as a foreign language sequence that the LLM can comprehend.
%enable multimodal understanding and generation with a frozen LLM.
We propose \emph{Semantic Pyramid AutoEncoder} (\modelname{}), a new tokenizer that converts between the raw signal and a lexical word sequence with dynamically adjusting length that 1) carries rich semantics and 2) retains fine details for signal reconstruction.
To work with a frozen LLM via in-context learning, we introduce a progressive in-context denoising method to facilitate generation of long cross-modal sequences.

\subsection{Semantic Pyramid AutoEncoder}
\label{sec:tokenizer}
\vspace{-3mm}

\begin{figure}
%{r}{0.5\textwidth}
\vspace{-5mm}
\centering
\includegraphics[width=0.5\columnwidth]{figures/framework.pdf}
\caption{Framework of the proposed \modelname{} model.}
\label{fig:framework}
\vspace{-3mm}
\end{figure}

Our \modelname{} model is built upon the VQVAE~\cite{van2017neural} framework.
%given its high reconstruction fidelity across different modalities.
We take the image modality below to introduce our \modelname{} model in a 2D case, as illustrated in~\cref{fig:framework}.
\modelname{} generates lexical tokens arranged in a pyramid structure, which contains semantics in the upper layers and as well as appearance with progressively refined details in the lower layers. 
%\lu{figure does not draw the progressive part and semantic meaning.}

\vspace{-4mm}
\paragraph{Frozen language codebook.}
%A standard VQGAN model jointly learns the VQ codebook with the encoder and decoder stacks through a dictionary learning objective~\cite{van2017neural}.
%Therefore, tokens from a VQGAN are not directly interpretable in natural languages.
To produce tokens in the lexical space, we use a frozen codebook $\sC = \{(k, \rve(k)) \mid k \in \sT\}$ where $\sT$ is the vocabulary of a pretrained LLM.
%
$\rve(\cdot)$ produces a text embedding vector for each sub-word token, which may be obtained either from the LLM's input embeddings or from the embeddings in subsequent layers.
%as in LQAE~\cite{liu2023language} 


% Lu: add this to the supplementary materials
% \begin{wrapfigure}{r}{0.4\textwidth}
% \vspace{-5mm}
% \centering
% \includegraphics[width=0.4\columnwidth,trim={0 0 0 0},clip]{figures/dilation_sampler.pdf}
% \vspace{-5mm}
% \caption{Dilation subsampler.}
% \label{fig:dilation}
% \vspace{-5mm}
% \end{wrapfigure}

\vspace{-4mm}
\paragraph{Token pyramid.}
\modelname{} encodes an image $\rmI \in \sR^{H \times W \times 3}$ into latent embeddings $\rmZ \in \sR^{h_D \times w_D \times c}$.
The embeddings are quantized into $D$ layers of tokens $\{\rvk_l  \in \sT^{h_l \times w_l} \mid l \in [1, 2, \hdots, D]\}$, with the constraint $h_l \le h_{l+1} \land w_l \le w_{l+1}$ to form a pyramid structure. 
%with enforce $h_l \le h_{l+1} \land w_l \le w_{l+1}$ to form a token pyramid.


The pyramid structure is important not only in tokenizing the input with a dynamically adjusting length, suitable for diverse tasks, but also concentrating semantics in the top pyramid layers, represented by fewer tokens.
\kevin
{It is unclear if the spatial arrangment of tokens is related to the spatial structure of the image, or is just a bag of tokens at each layer.
I think what you are doing is partitioning all the discrete tokens into a set of sets,
with $D$ outer sets,
and each inner set for each layer $l$.
}
\lijun{Based on empirical results, tokens from convolution-based VQVAE have spatial correspondence with the image patches, but I think this is irrelevant to what we are trying to describe here.
The tokens are in an ordered list of sets, with each set for each layer $l$, and deeper layers could depend on the previous ones, both in RQ and SAQ.
} \lu{I think this is implicitly stated as each layer follows the VQVAE token structure.}

%layers in monotonically increasing sizes. This structure concentrates high level concepts in the shallow layers with fewer tokens, while appearance details are preserved in deeper layers.
%\cref{fig:dilation} illustrates the formation of
%the pyramid with 
A dilation subsampler $\rmP(l)$ is used, which selects the positions for quantization at layer $l$ as
\vspace{-2mm}
\begin{equation}
    \rmP(l) = \{(h'i - \left\lceil\frac{h'}{2}\right\rceil + 1, w'j - \left\lceil\frac{w'}{2}\right\rceil + 1) \mid (i, j) \in ([1, h_l] \times [1, w_l]) \cap \sZ^2  \}
\end{equation}
where $h'=\frac{h_D}{h_l}$, and $w'=\frac{w_D}{w_l}$ are the downsample ratios.

% \begin{wrapfigure}{r}{0.4\textwidth}
% \vspace{-5mm}
% \centering
% \includegraphics[width=0.4\columnwidth,trim={0 0.4cm 0 0.4cm},clip]{figures/saq_vs_rq.pdf}
% \vspace{-5mm}
% \caption{Comparison between RQ and SAQ.}
% \vspace{-3mm}
% \label{fig:saq}
% \end{wrapfigure}

\vspace{-4mm}
\paragraph{Streaming average quantization.}
Residual Quantization (RQ) is commonly used to produce multi-layer tokens in image and audio models~\cite{lee2022autoregressive,zeghidour2021soundstream}, where all layers are of the same shape.
% For each latent position, the token at layer $l$ is quantized from
% \begin{equation}
%     \rvz_l = \rvz - \textstyle \sum_{i=1}^{l-1}\rve(k_i)
% \end{equation}
% The embedding up to layer $l$ is reconstructed as
% \begin{equation}
%     \rvz'_l = \textstyle \sum_{i=1}^{l}\rve(k_i)
% \end{equation}
RQ is sub-optimal for \modelname{} with a frozen language codebook, in part because
(1) RQ negatively affects the code utilization rate because embeddings in different residual layers are at different scales, which could divide the codebook into multiple parts;
(2) summation of word embeddings is not well aligned, which limits the presence of semantically meaningful tokens in later layers.
To tackle these issues, we introduce Streaming Average Quantization (SAQ)
\kevin{What does streaming mean?}
to produce multi-layer tokens in variable shapes.
For each latent position $(x, y)$,
\kevin{
This is unclear.
I thought you learned a bag of codewords for the entire image? Where does spatial locality come in? 
}
the SAQ token at layer $l$ is selected as $k_{(l, x, y)} = \argmin_{k \in \sT}\|\rvz_{(l, x, y)} - \rve(k)\|_2^2$ with embedding
\vspace{-1mm}
\begin{equation}
    \rvz_{(l, x, y)} = \rvz_{(x, y)} + \textstyle \sum_{i=1}^{l-1}\1_{(x, y) \in \rmP(i)}(\rvz_{(x, y)} - \rve(k_{(i, x, y)}))
\end{equation}
\kevin{Should this be $\hat{z}_{lxy}$ on LHS?} \lijun{This is pre-quantization embedding, but I agree with the suggestion below to define a reconstruction function for clarity}
% \lu{P(i) not defined} % lijun: it's eq(1)
where $\1$ is the indicator function. 

The decoder reconstructs taking the input of $\hat{\rmZ}(l)$, up to layer $l$,
\vspace{-1mm}
\begin{equation}
    \hat{\rvz}_{(l, x, y)} = \frac{\sum_{i=1}^{l}\1_{(x, y) \in \rmP(i)}\rve(k_{(i, x, y)})}{\sum_{i=1}^{l}\1_{(x, y) \in \rmP(i)}}
\end{equation}
\kevin{ It would be clearer to define the reconstruciton as a function $\hat{z} =  r(z) = r'(k(z))$, which takes the continuous encoding $z$, maps it to discrete codewords $k(z)$,
and then reconstructs by doing spatial averaging.
}


SAQ takes a streaming average of the embeddings, which dynamically simulates a bag-of-words representation.
Variable layer shapes are supported by skipping early quantization steps when a position is only present in later layers.

\vspace{-4mm}
\paragraph{Semantic guidance.}
We encourage the semantic similarity between the input image $\rmI$ and each produced lexical token $k$ by $s(\rmI, k)$.
During training, we build per-layer candidate token pools as
\vspace{-1mm}
\begin{equation}
    \rmC_l(\rmI) = \{k \in \sT \mid s(\rmI, k) \ge \rho_l\}
\end{equation}
where $\rho_l$ is a threshold hyperparameter.
We set $\rho_l \ge \rho_{l+1}$ to allow for more candidates in deeper layers with more tokens.
Given an embedding $\rvz$ \in $\rmZ$, a single-step quantizer~\cite{van2017neural} computes the L2 distances between $\rvz$ and all entries in $\sC$.
We take the opposite of the distances as logits and apply a cross entropy loss towards a target code randomly sampled from the candidate pool, calculated from: 
\vspace{-1mm}
\begin{equation}
    \gL_\mathit{semantic}(\rmI) = \mathop{\E}\limits_{l \in [1, D]}\mathop{\E}\limits_{\rvz_l}\mathop{\E}\limits_{c \sim \rmC_l(\rmI)} -\log \frac{\exp(-\|(\rvz_l - \rve(c)\|^2_2)}{\sum_{k \in \sT} \exp(-\|\rvz_l - \rve(k)\|^2_2)}
\end{equation}
% \lu{d should be D in Eq 3?}
\kevin{It is not clear what parameters this loss function depends on. e() is frozen, so is
$z_l = g(I; \theta)$ the learned encoder?
If so, write $L(\theta;I)$.
}
\lijun{Yes it's depending on the encoder. But it is a little tricky to expand $z_l$ with $g(I; \theta)$ for $l > 1$, which will become eq (2)}

% \vspace{-4mm}
% \paragraph{Semantic similarity guidance.}
% \kevin{Move this earlier, right after eqn 2}
Using image-text pairs~\cite{liu2022cross} in training could lead to a golden definition of $s(\rmI, k)$, but it limits the potential usage of large-scale unpaired data.
In this work, we capture the similarity using a pretrained cross-modal embedding model, such as CLIP~\cite{radford2021learning}, and train with image/video data without text descriptions.
Let $f_\gI$ and $f_\gT$ be a pair of image and text encoders mapping into a shared space.
We precompute the text feature for each lexical token $k \in \sT$ as
\vspace{-1mm}
\begin{equation}
    f'_\gT(k) = \frac{1}{|\rvp|} \textstyle \sum_{i=1}^{|\rvp|} f_\gT(\ervp_i(k))
\end{equation}
where $\rvp$ is a list of prompt templates, such as \texttt{"a photo of ..."}.
During training, we extract the image feature $f_\gI(\rmI)$ and compute the raw similarity scores as
\begin{equation}
    \rvs'(\rmI, k) = f_\gI(\rmI) \cdot f'_\gT(k)
\end{equation}
The similarity score is then normalized to account for the varying scales across different images.
%scale of the similarity scores varies by image, so we use the relative score as the final measurement:
\begin{equation}
    \rvs(\rmI, k) = \frac{\rvs'(\rmI, k) - \textstyle \min_j \rvs'(\rmI, j)}{\max_j \rvs'(\rmI, j) - \min_j \rvs'(\rmI, j)} \label{eq:relative_clip}
\end{equation}
\vspace{-4mm}
\paragraph{Training.}
Following an improved VQGAN objective in~\cite{yu2022magvit}, the appearance losses calculate from:

\vspace{-2mm}
\begin{equation}
    \gL_\mathit{appearance}(\rmI) = \|\rmI - \hat{\rmI}\|_2^2 + \beta \textstyle \sum_{l=1}^D\|\rmZ - \hat{\rmZ}_l\|_2^2 + \lambda \gL_\mathit{GAN} + \eta \gL_\mathit{Perceptual},
\end{equation}
\kevin{How is $\hat{I}$ computed?
Why do you care about reconstruction accuracy of $\hat{Z}$?
}
where $\gL_\mathit{GAN}$ and $\gL_\mathit{Perceptual}$ are the VQGAN~\cite{ge2022long} and perceptual loss~\cite{johnson2016perceptual}. The codebook learning loss is dropped given the frozen codebook.

To stabilize the training and balance between appearance and semantics, we adopt a dynamic weight for the semantic guidance loss.
The total training loss excluding the discriminator part is
\begin{equation}
    \gL_\mathit{\modelname{}} = \mathop{\E}\limits_{\rmI} \Big[\gL_\mathit{appearance}(\rmI) + \alpha \text{sg}\Big(\frac{\gL_\mathit{appearance}(\rmI)}{\gL_\mathit{semantic}(\rmI)}\Big)\gL_\mathit{semantic}(\rmI)\Big],
\end{equation}
where $\text{sg}[\cdot]$ is the stop-gradient operation.
\kevin{This is confusing. You put an sg on the first term but not the second, so you will still end up taking gradients wrt both losses.
}
% During decoding, quantized embeddings $\rmX' \in \sR^{h_k \times w_k}$ can be constructed with the first $k \le d$ levels of tokens, which is then decoded into the pixel space.
 


% \subsubsection{Loss}

% It is worth noting that \modelname{} is trained standalone without back propagation through any language model, which is different from LQAE and Frozen~\cite{tsimpoukelli2021multimodal}.

\subsection{Progressive In-Context Denoising}
\label{sec:prompting}
While our method is the most effective when backpropagating through LLMs by prompt~\cite{lester2021power} or adapter tuning, this paper focuses on verifying its plausibility in an extreme setting of in-context learning.
We demonstrate that LLMs are capable of performing new tasks in foreign modalities without any parameter updates.
%While our method is best with updating the parameters LLMs through back propagation such as finetuning or prompt tuning, LoRA, 
% We adopt the in-context learning~\cite{brown2020language} framework for multimodal understanding and generation tasks with LLMs without parameter updates.
Specifically, a set of $K$ examples $\{(\rvu^i, \rvv^i)\}_{i=1}^K$ are fed to the LLM to learn a new task and answer a query $\hat{\rvu}$ with
\vspace{-1mm}
\begin{equation}
    \hat{\rvv} \sim \pllm(\cdot | \hat{\rvu}; \{(\rvu^i, \rvv^i)\}_{i=1}^K) \label{eq:icl}
\end{equation}

Sampling $\hat{\rvv}$ by autoregressive decoding is suboptimal due to the distributional discrepancy in the representation and the presence of exceptionally long sequences, \eg, an image is quantized into over 500 words. 
% It is straightforward to generate textual $\hat{\rvv}$ in a single pass of autoregressive decoding, where the LLM has a strong prior about the output distribution.
% However, token sequences from foreign modalities have much smaller likelihoods in the LLM due to the distribution difference and the greater lengths.
To this end, we introduce a progressive in-context denoising method.
%to effectively generate such sequences.

\vspace{-4mm}
\paragraph{Progressive generation.}
We generalize \cref{eq:icl} into a multi-step generation process.
Let $s_t$ denote the number of tokens generated in $t$ steps.
At each step, we sample a sub-sequence
\begin{equation}
    \hat{\rvv}_{s_t:s_{t+1}} \sim \pllm(\cdot | [\hat{\rvu}, \hat{\rvv}_{< c_t}]; \{([\rvu^i, \rvv^i_{< c_t}], \rvv^i_{s_t:s_{t+1}})\}_{i=1}^K)
\end{equation}
where $[\cdot, \cdot]$ concatenates the sequences and $c_t$ controls the length of previous outputs to condition on.
\kevin{This is very unclear}
When $c_t=s_t$, it is an autoregressive (AR) process, where the later tokens condition on all previous tokens.
When $c_t=0$, it corresponds to a non-autoregressive (NAR) process, where each sub-sequence $\hat{\rvv}_{s_t:s_{t+1}}$ is sampled independently.
% \lu{still depend on $\rvv^i_{s_t:s_{t+1}})$?} %lijun: yes because it's generating this segment; but it's not dependent on $\rvv^i_{<s_t}$.
In a more general setup, we use AR for the first $T'$ steps and NAR for the remains, which follows $c_t = \min(s_t, s_{T'})$.

\vspace{-4mm}
\paragraph{In-context denoising.}
The learning capacity of an in-context setup is far from sufficient for the entirety of a foreign modality $\gM$.
Therefore, we operate in a denoising subspace to achieve effective generation.
\kevin{This is best explained by referring to an example image}
Take an image-to-image task as example.
Examples are created based on a subset of real images $\gM'$ and a token-space random corruption function $\epsilon(\cdot; r)$, where the corruption ratio $r$ follows a predefined schedule.
\begin{equation}
    (\rvu^i, \rvv^i) \sim \Big(\epsilon\big(\mathit{\modelname{}}(\eta(\rmI)); r_i\big), \epsilon\big(\mathit{\modelname{}}(\rmI); r_i\big)\Big), \rmI \in \gM' \subset \gM
\end{equation}
\kevin{This is very hard to read; define dummy variables}
where $\eta$ is a pixel-space task-specific function to create the condition image, such as masking out the bottom half for out-painting.
The query $\hat{\rvu}$ is always sampled from $\gM'$ without noise, where we ensure $\epsilon$ is never an identity mapping to avoid information leakage.
When $|\gM'|=1$, this forms a denoising image generation model from a single image.

% In-context learning~\cite{brown2020language} is an approach to leveraging LLMs to quickly learn a new task with a few examples. LLMs are usually prompted with a set of input-output pairs (i.e., $K$-shot prompting)  to demonstrate the target task. A test input $\hat{\rvu}$ follows the $K$-shot prompt to ask the model to predict the output $\hat{\rvv}$ conditioning on the prompt $\mathcal{P}$ and test input $\hat{\rvu}$. Due to the effectiveness without optimizing any parameters, we utilize this method to verify our \modelname{} on different downstream tasks. However, it is challenging for LLMs to directly output the sequence of semantic language tokens for images/videos in a single pass as the LLMs have never seen these kinds of sequences in pre-training. To lessen the workload of LLMs in predicting an entire sequence in a single step, we propose a decoding method called \emph{Progressive Prompting} by breaking down the single-step prompting and prediction into multiple steps with a stride of $s$:

% A sequence of the same size as output in the prompt is generated as the latent codebook ids for the test input. To speed up few-shot inference while keeping the high-quality prediction, we strike a balance to decode $s$ tokens with the conventional autoregressive decoding each time. 
% % Thus we can finish the generation within $\left\lceil\frac{|t|}{k}\right\rceil$ steps.


==> tables/miniimagenet_5way.tex <==
\begin{table}[tp]
% \vspace{-6mm}
\centering
\caption{\textbf{Few-shot classification accuracy} on the mini-ImageNet 5-way benchmarks.}
\label{tab:imagenet_5way}
\small
\begin{tabular}{@{}lllcccccccc@{}}
\toprule
\multicolumn{3}{r}{Task Induction} & & \checkmark & \checkmark& \checkmark& \checkmark& \checkmark& \checkmark & \multirow{3}{*}{Avg} \\
Method  &\# Layers & \multicolumn{1}{r}{Inner Shots}    & 1            & 1             & 3             & 5             & 1             & 1             & 1             &                      \\
& : \# Tokens & \multicolumn{1}{r}{Repeats}        & 0            & 0             & 0             & 0             & 1             & 3             & 5             &                      \\ 
\midrule
Frozen~\cite{tsimpoukelli2021multimodal} &- &     & 0.9          & 14.5          & 34.7          & 33.8          & 33.8          & 33.3          & 32.8          & 26.26                \\ \midrule
LQAE~\cite{liu2023language} & 1: 256 & GPT 3.5 & 1            & 15.7          & 35.9          & 36.5          & 31.9          & 36.4          & 45.9          & 29.04                \\
$\emph{\modelname{}}_\text{GPT}$ (ours) &2: 5& GPT 3.5 & \textit{4.3} &  \textit{63.0}    &   \textit{63.4}   &    \textit{60.6}  & \textit{61.9} & \textit{62.1}  & \textit{62.1}    &    \textit{53.91}                  \\ \midrule
$\emph{\modelname{}}_\text{PaLM}$ (ours) & 2: 5  & PaLM 2     & \textbf{23.6} & 64.2 & 68.0 & 69.9 & 63.4 & 62.0 & 60.2 & 58.76       \\ 
$\emph{\modelname{}}_\text{PaLM}$ (ours) & 3: 21 & PaLM 2     & 20.2 & \textbf{65.1} & \textbf{73.7} & \textbf{74.3} & \textbf{66.4} & \textbf{67.0} & \textbf{66.3} & \textbf{61.86}       \\ 
% & \makecell[r]{$d=$} & $1$ & $3$ & $3$ & $3$ & $3$ & $3$ & $4$ \\ 
\bottomrule
\end{tabular}
\vspace{-4mm}
\end{table}

==> tables/miniimagenet_5way_full.tex <==
\begin{table}[tp]
% \vspace{-6mm}
\centering
\caption{\textbf{Few-shot classification accuracy} on the mini-ImageNet 5-way benchmarks. - means value unavailable due to an infeasible sequence length.}
\label{tab:imagenet_5way_full}
% \small
\begin{tabular}{@{}lllcccccccc@{}}
\toprule
\multicolumn{3}{r}{Task Induction} & & \checkmark & \checkmark& \checkmark& \checkmark& \checkmark& \checkmark & \multirow{3}{*}{Avg} \\
Method  &\# Layers & \multicolumn{1}{r}{Inner Shots}    & 1            & 1             & 3             & 5             & 1             & 1             & 1             &                      \\
& : \# Tokens & \multicolumn{1}{r}{Repeats}        & 0            & 0             & 0             & 0             & 1             & 3             & 5             &                      \\ 
\midrule
% Frozen~\cite{tsimpoukelli2021multimodal} &- &     & 0.9          & 14.5          & 34.7          & 33.8          & 33.8          & 33.3          & 32.8          & 26.26                \\
LQAE~\cite{liu2023language} & 1: 256 & GPT 3.5 & 1            & 15.7          & 35.9          & 36.5          & 31.9          & 36.4          & 45.9          & 29.04                \\ \midrule
% \emph{\modelname (Ours)} & GPT-3.5 &              &               &               &               &               &               &               &                      \\
\emph{\modelname{}}$_\text{PaLM}$ & 1: 1  & PaLM 2     & \textbf{26.8} & 52.0 & 50.9 & 49.9 & 51.9 & 48.4 & 47.9 & 46.83       \\ 
\emph{\modelname{}}$_\text{PaLM}$  & 2: 5  & PaLM 2     & 23.6 & 64.2 & 68.0 & 69.9 & 63.4 & 62.0 & 60.2 & 58.76       \\ 
\emph{\modelname{}}$_\text{PaLM}$  & 3: 21 & PaLM 2     & 20.2 & \textbf{65.1} & \textbf{73.7} & \textbf{74.3} & \textbf{66.4} & \textbf{67.0} & 66.3 & \textbf{61.86}       \\ 
\emph{\modelname{}}$_\text{PaLM}$  & 4: 85  & PaLM 2     & 16.1 & 58.5 & 67.2 & 69.1 & 64.0 & 66.4 & \textbf{67.4} & 58.39       \\ 
\emph{\modelname{}}$_\text{PaLM}$  & 5: 341  & PaLM 2     & 12.1 & 46.3 & 55.9 & 67.2 & 43.3 & 46.3 & - & -      \\ 
\emph{\modelname{}}$_\text{PaLM}$  & 6: 597  & PaLM 2     & 12.1 & 35.7 & - & - & - & - & - & -      \\ 
%\midrule
%\emph{\modelname{}}$_\text{PaLM}^\text{clean}$  & 2: 5 & PaLM 2   & 13.6 & 56.4 & 59.2 & 60.0 & 54.2 & 50.2 & 48.1 & 48.82 \\
%\emph{\modelname{}}$_\text{PaLM}^\text{clean}$  & 3: 21 & PaLM 2   & 10.4 & 57.3 & 62.1 & 62.8 & 56.9 & 55.2 & 51.6 & 50.90 \\
% & \makecell[r]{$d=$} & $1$ & $3$ & $3$ & $3$ & $3$ & $3$ & $4$ \\ 
\bottomrule
\end{tabular}
% \vspace{-4mm}
\end{table}
